COVID-19: Social Media Sentiment Analysis on Reopening

The novel coronavirus (COVID-19) pandemic is the most talked topic in social media platforms in 2020. People are using social media such as Twitter to express their opinion and share information on a number of issues related to the COVID-19 in this stay at home order. In this paper, we investigate the sentiment and emotion of peoples in the United States on the subject of reopening. We choose the social media platform Twitter for our analysis and study the Tweets to discover the sentimental perspective, emotional perspective, and triggering words towards the reopening. During this COVID-19 pandemic, researchers have made some analysis on various social media dataset regarding lockdown and stay at home. However, in our analysis, we are particularly interested to analyse public sentiment on reopening. Our major finding is that when all states resorted to lockdown in March, people showed dominant emotion of fear, but as reopening starts people have less fear. While this may be true, due to this reopening phase daily positive cases are rising compared to the lockdown situation. Overall, people have a less negative sentiment towards the situation of reopening.

==> trash/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
Emotions and sentiments are the driving force that people are sharing in social media. If we analyze the social media posts then we can find the insights of those posts along with emotions and sentiments. From this kind of analysis, we may find what people like, what they want, and what are the main concerns of them.
Our analysis is to help people around the world through posts related to COVID-19.
Coordination of responses from online and from the real-world is sure to reveal promising results to address the current crisis. We want to put stress on the fact that along with traditional public health surveillance, infoveillance studies can play a vital role. In addition, even though the peoples are protesting to reopen their areas and economy but actually without proper precautions it is very dangerous. From real-world data we saw that reopen may increase the new cases. That's why state organizations and health organizations need to spread the proper pieces of information and guidelines, they need to take proper actions to reduce the new cases. Also, people need to follow the guidelines properly because with proper steps and precautions we can win over this pandemic.


\Part{Source Code.} We have released the source code for public dissemination and can be found at https://github.com/emtiaz-ahmed/COVID19-Twitter-Reopen.


==> trash/emotone.tex <==
\begin{figure*} [h!]
\noindent \begin{minipage}{.5\textwidth}

\includegraphics[width=0.99\linewidth]{figs/tone_perc_time.png}
\caption*{(a) Emotional Tone}
\end{minipage}%
\begin{minipage}{.5\textwidth}

\includegraphics[width=0.99\linewidth]{figs/uttr_perc_time.png}
\caption*{(b) Emotional Utterance}
\end{minipage}
\caption{Number of tweet (\%) over date.}
\label{fig:emotion_perc_time}
\end{figure*}


==> trash/emouttr.tex <==
\begin{figure*} [h!]
\noindent \begin{minipage}{.5\textwidth}
\includegraphics[width=0.99\linewidth]{figs/tone_perc_type.png}
\caption*{(a) Emotional Tone}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\includegraphics[width=0.99\linewidth]{figs/uttr_perc_type.png}
\caption*{(b) Emotional Utterance}
\end{minipage}
\caption{Number of tweet (\%) across emotion types.}
\label{fig:emotion_perc_type}
\end{figure*}


==> trash/texxuttr.tex <==
\subsection{Emotion Analysis}
\label{sec:methodology_emotion}
We used the \texttt{Python} implementation of IBM Watson™ Tone Analyzer service \footnote{\url{https://cloud.ibm.com/apidocs/tone-analyzer?code=python}} to detect emotional tones and utterances in tweets. The emotion of tweet is analyzed in two perspectives: (1) ToneAnalyses, and (2) UtteranceAnalyses. The \texttt{ToneAnalyses} API uses the general-purpose endpoint to analyze the tone of a tweet, and reports the following tones: analytical, tentative, confident, joy, fear, sadness, and anger. On the other hand, the \texttt{UtteranceAnalyses} API uses the customer-engagement endpoint to analyze the utterance of a tweet, and reports the following tones: sad, frustrated, satisfied, excited, polite, impolite, and sympathetic. The emotion detection process is summarized as following steps: 
\smallskip
\begin{itemize} [nosep]
\item Create a Tone Analyzer service in IBM Cloud for a specific region and API plan.
\item Get the API key, the service endpoint URL, and the version of API.
\item Authenticate to the API using IBM Cloud Identity and Access Management (IAM).
\item Request up to $100$ sentences (no more than $128$ KB size in total) for the sentence-level tone analysis, and up to $50$ sentences (no more than $500$ characters for each sentence) for the utterance analysis.
\item Parse the JSON responses that provide the results for each tone and utterance of the tweet.
\end{itemize}
\smallskip
Note that, in our analysis, the \texttt{ToneAnalyses} requires a tweet as a single sentence for detecting sentence-level emotional tones, and the \texttt{UtteranceAnalyses} uses $500$ characters of a tweet for detecting emotional utterances. 

